The Hessian perspective into the Nature of Convolutional Neural Networks

While Convolutional Neural Networks (CNNs) have long been investigated and applied, as well as theorized, we aim to provide a slightly different perspective into their nature -- through the perspective of their Hessian maps. The reason is that the loss Hessian captures the pairwise interaction of parameters and therefore forms a natural ground to probe how the architectural aspects of CNN get manifested in its structure and properties. We develop a framework relying on Toeplitz representation of CNNs, and then utilize it to reveal the Hessian structure and, in particular, its rank. We prove tight upper bounds (with linear activations), which closely follow the empirical trend of the Hessian rank and hold in practice in more general settings. Overall, our work generalizes and establishes the key insight that, even in CNNs, the Hessian rank grows as the square root of the number of parameters.

==> archived.tex <==
\section{Rank comparisons at equal parameter budget}
To ground our comparisons, we will now assume that we are given a particular parameter budget $p$, and we are required to design the network architecture, in particular choose number of channels (or neurons) $m$ and kernel size $k$, for these three kinds of architectures. 

For the FCN, number of neurons is considered to be $M_{F} = m_F \dfrac{d}{k}$. For the same number of parameters, the LCN can have $m_L = m_F \cdot \dfrac{d+K}{k+K}$ channels, while the CNN can have $m_L = m_F \cdot \dfrac{d^2+Kd}{k^2+Kd}$. Note, to compare, we will chose such a value of $m_F$ so that $m_L, m_C$ come out as integers. Now, let us contrast their Hessian ranks. 

\textcolor{red}{See if there's actual value of doing this exercise. Maybe the correlation study? Especially, given things change when $K> 1$}
\subsubsection{When $K=1$.} 
As a starting point, to simplify comparisons, we assume the number of outputs, $K=1$. Since $K=1$, the outer-product Hessian has the same rank in these scenarios. Thus the overall Hessian rank will be largely determined by the rank of the functional Hessian, except for additive constants. So, let us compare the rank of the functional Hessians then. First, for FCN, we 
 will have:
\[\rank(\HFsup{\text{FCN}}) = 2m_F \cdot \dfrac{d}{k}\]
Whereas, for the case of LCN, we obtain:
\[\rank(\HFsup{\text{LCN}}) = 2m_F \cdot \dfrac{d}{k}\cdot \dfrac{d+1}{k+1}\]

Lastly, for the CNN case, we get:
\begin{align*}
\rank(\HFsup{\text{CNN}}) &= 2m_F \cdot \dfrac{d^2+d}{k^2+d} \cdot \min\left(k, \dfrac{d}{k}\right)=2m_F \cdot \dfrac{d}{k}\cdot \dfrac{d+1}{k+ d/k}\cdot \min\left(k, \dfrac{d}{k}\right)\\
\end{align*}

\paragraph{When $d\geq k\geq d^{\frac{1}{3}}$} 
Here, we obtain:
\[\rank(\HFsup{\text{CNN}})\geq \rank(\HFsup{\text{LCN}}) \geq \rank(\HFsup{\text{FCN}})\,.\]
\paragraph{When $d^{\frac{1}{3}}\geq k\geq 1$} 
In this scenario, the LCN actually exceeds CNN in terms of the functional Hessian rank. More concretely, it can be shown that:
\[\rank(\HFsup{\text{LCN}})\geq \rank(\HFsup{\text{CNN}}) \geq \rank(\HFsup{\text{FCN}})\,.\]

We show the empirical evidence for this, in the case of linear as well as non-linear activations, in the Figures~\ref{fig:rank-cnn-lcn-fcn-linear} and~\ref{fig:rank-cnn-lcn-fcn-relu} respectively.

\begin{proof}
\textit{Comparing CNN and FCN}:
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} &= \dfrac{2m_F \cdot \dfrac{d^2+d}{k^2+d} \cdot \min\left(k, \dfrac{d}{k}\right)}{2 \, m_F \cdot \dfrac{d}{k}}= \dfrac{kd^2+kd}{d^2 + k^2d} \cdot \min\left(k, \dfrac{d}{k}\right)\\
\end{align*}
When $k\leq \dfrac{d}{k}$, we get that: 
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})}& = \dfrac{k^2d^2+k^2d}{d^2 + k^2d} \geq 1 \\
\end{align*}
When $k\geq \dfrac{d}{k}$, we get that: 
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})}& = \dfrac{d^2+d}{k^2 + d} \geq 1 \\
\end{align*}
\end{proof}

\subsubsection{Beyond $K=1$} 
The whole picture becomes more nuanced when we consider $K>1$.

\paragraph{Comparing CNN and FCN}
What we will find it that as long as $K\geq \dfrac{k^2}{d}$, it is in fact the FCN which has higher functional Hessian rank than the CNN. But when $1\leq K \leq \dfrac{k^2}{d}$, we have it the other way around which also matches the prediction from $K=1$ analysis before. 
\begin{proof}
The general expression of the ratio of the functional Hessian ranks for CNN and FCN is as follows:
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} &= \dfrac{2m_F \cdot \dfrac{d^2+Kd}{k^2+Kd} \cdot \min\left(k, \dfrac{Kd}{k}\right)}{2 \, m_F \cdot \dfrac{d}{k} \min(K, d)} = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{\min\left(k^2, Kd\right)}{\min\left(d^2, Kd\right)}\\
\end{align*}

Case 1: When $K\geq d$. In this case, although this is not as likely in practice, we have that $\rank(\HFsup{\text{CNN}})\leq \rank(\HFsup{\text{FCN}})$.

\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{k^2}{d^2}= \dfrac{d^2k^2 + Kdk^2}{d^2k^2 + Kd^3} \leq 1\,.
\end{align*}

Case 2: When $k \leq K\leq d$. 
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{k^2}{Kd}= \dfrac{k^2 d^2 + Kdk^2}{K^2d^2 +Kdk^2 } \leq 1\,.
\end{align*}

Case 3: When $\dfrac{k^2}{d} \leq K\leq k$. This leads to the same outcome as the case 2.
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{k^2}{Kd}= \dfrac{k^2 d^2 + Kdk^2}{K^2d^2 +Kdk^2 } \leq 1\,.
\end{align*}

Case 4: When $1\leq K\leq \dfrac{k^2}{d}$. 
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{Kd}{Kd}= \dfrac{d^2 + Kd}{k^2 +Kd } \geq 1\,.
\end{align*}
\end{proof}
% When $1\leq k\leq \sqrt{Kd}$, we obtain:
% \begin{align*}
% \dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} 
% & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{k^2}{\min\left(d^2, Kd\right)}\\
% \end{align*}

% When $d\geq k\geq \sqrt{Kd}$, we obtain:
% \begin{align*}
% \dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{FCN}})} 
% & = \dfrac{d^2+Kd}{k^2 + Kd} \cdot \dfrac{Kd}{\min\left(d^2, Kd\right)}\\
% \end{align*}

\paragraph{Comparing LCN and FCN.}

For LCN, it is a bit more nuanced. When $K\geq \sqrt{kd}$, $\rank(\HFsup{\text{FCN}})\geq \rank(\HFsup{\text{LCN}})$. But when $K\leq \sqrt{kd}$, then $\rank(\HFsup{\text{LCN}})\geq \rank(\HFsup{\text{FCN}})$.

\begin{proof}
\begin{align*}
\dfrac{\rank(\HFsup{\text{LCN}})}{\rank(\HFsup{\text{FCN}})} &= \dfrac{2 \, m_F \cdot \dfrac{d+K}{k+K} \cdot \dfrac{d}{k} \cdot \min\left(k, K\right)}{2m_F \cdot \dfrac{d}{k} \cdot \min\left(K, d\right)}=\dfrac{d+K}{k+K}\cdot \dfrac{\min\left(K, k\right)}{\min\left(K, d\right)}\\
\end{align*}

Case 1: When $K\geq d$,

\begin{align*}
\dfrac{\rank(\HFsup{\text{LCN}})}{\rank(\HFsup{\text{FCN}})} & =\dfrac{d+K}{k+K}\cdot \dfrac{k}{d} = \dfrac{kd+ Kk}{kd + Kd}\leq 1\\
\end{align*}

Case 2: When $d\geq K\geq \sqrt{kd}$,
\begin{align*}
\dfrac{\rank(\HFsup{\text{LCN}})}{\rank(\HFsup{\text{FCN}})} & =\dfrac{d+K}{k+K}\cdot \dfrac{k}{K} = \dfrac{kd+ Kk}{K^2 + Kk }\leq 1\\
\end{align*}

Case 3: When $\sqrt{kd}\geq K\geq 1$,
\begin{align*}
\dfrac{\rank(\HFsup{\text{LCN}})}{\rank(\HFsup{\text{FCN}})} & =\dfrac{d+K}{k+K}\cdot \dfrac{k}{K} = \dfrac{kd+ Kk}{K^2 + Kk} \geq 1\\
\end{align*}
\end{proof}



\paragraph{Comparing CNN and LCN.}

For $K \geq  \sqrt{\dfrac{k^3}{d}}$, $\rank(\HFsup{\text{LCN}})\geq \rank(\HFsup{\text{CNN}})$; while for $K \leq  \sqrt{\dfrac{k^3}{d}}$, we have the reverse, i.e., $\rank(\HFsup{\text{CNN}})\geq \rank(\HFsup{\text{LCN}})$.
\begin{proof}
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{LCN}})} &= \dfrac{2m_F \cdot \dfrac{d^2+Kd}{k^2+Kd} \cdot \min\left(k, \dfrac{Kd}{k}\right)}{2 \, m_F \cdot \dfrac{d+K}{k+K} \min\left(d, \dfrac{Kd}{k}\right)}=\dfrac{kd + Kd }{k^2 + Kd}\cdot \dfrac{\min(k^2, Kd)}{\min(kd, Kd)}\\
\end{align*}
Case 1: When $K\geq k$:
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{LCN}})} & =\dfrac{kd + Kd }{k^2 + Kd}\cdot \dfrac{k^2}{kd}=\dfrac{k^2+Kk}{k^2 + Kd}\leq 1
\end{align*}

Case 2: When $k \geq K \geq \sqrt{\dfrac{k^{3}}{d}}$
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{LCN}})} & =\dfrac{kd + Kd }{k^2 + Kd}\cdot \dfrac{k^2}{Kd}=\dfrac{k^3+Kk^2}{K^2 d + Kk^2}\leq 1
\end{align*}

Case 3: When $\sqrt{\dfrac{k^{3}}{d}} \geq K \geq \dfrac{k^2}{d}$
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{LCN}})} & =\dfrac{kd + Kd }{k^2 + Kd}\cdot \dfrac{k^2}{Kd}=\dfrac{k^3+Kk^2}{K^2 d + Kk^2}\geq 1
\end{align*}

Case 4: When $\dfrac{k^2}{d}\geq K \geq 1$
\begin{align*}
\dfrac{\rank(\HFsup{\text{CNN}})}{\rank(\HFsup{\text{LCN}})} & =\dfrac{kd + Kd }{k^2 + Kd}\cdot \dfrac{Kd}{Kd} \geq 1
\end{align*}
\end{proof}



\begin{figure}[!t]
    \centering
    \begin{subfigure}{\textwidth}
    \includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/linear_param_budget/cnn.png}
    % \caption{CNN}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
\includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/linear_param_budget/lcn.png}
\end{subfigure}
    % \caption{LCN}
    % \caption{Effect of bias on $\effparams$ for varying depth}
    % % \label{fig:bias-a2}
    \begin{subfigure}{\textwidth}
\includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/linear_param_budget/fcn.png}
    % \caption{FCN}
    % \label{fig:bias-a2}
    \end{subfigure}
    \caption{\textit{For linear activations: }Comparison of the Functional Hessian spectrums of CNN, LCN, and FCN for networks where the number of parameters is same across the three architectures. }
    \label{fig:rank-cnn-lcn-fcn-linear}
\end{figure}

\begin{figure}[!t]
    \centering
    \begin{subfigure}{\textwidth}
    \includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/relu_param_budget/cnn.png}
    % \caption{CNN}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
\includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/relu_param_budget/lcn.png}
\end{subfigure}
    % \caption{LCN}
    % \caption{Effect of bias on $\effparams$ for varying depth}
    % % \label{fig:bias-a2}
    \begin{subfigure}{\textwidth}
\includegraphics[trim=20 20 50 39, clip, width=0.3\textwidth]{figures/relu_param_budget/fcn.png}
    % \caption{FCN}
    % \label{fig:bias-a2}
    \end{subfigure}
    \caption{\textit{For ReLU activations: }Comparison of the Functional Hessian spectrums of CNN, LCN, and FCN for networks where the number of parameters is same across the three architectures. }
\label{fig:rank-cnn-lcn-fcn-relu}
\end{figure}
